TorchDrug: A Powerful and Flexible Machine Learning Platform for Drug Discovery

Machine learning has huge potential to revolutionize the field of drug discovery and is attracting increasing attention in recent years. However, lacking domain knowledge (e.g., which tasks to work on), standard benchmarks and data preprocessing pipelines are the main obstacles for machine learning researchers to work in this domain. To facilitate the progress of machine learning for drug discovery, we develop TorchDrug, a powerful and flexible machine learning platform for drug discovery built on top of PyTorch. TorchDrug benchmarks a variety of important tasks in drug discovery, including molecular property prediction, pretrained molecular representations, de novo molecular design and optimization, retrosynthsis prediction, and biomedical knowledge graph reasoning. State-of-the-art techniques based on geometric deep learning (or graph machine learning), deep generative models, reinforcement learning and knowledge graph reasoning are implemented for these tasks. TorchDrug features a hierarchical interface that facilitates customization from both novices and experts in this domain. Tutorials, benchmark results and documentation are available at https://torchdrug.ai. Code is released under Apache License 2.0.

==> tables/graph_operation.tex <==
\begin{table}[!h]
    \centering
    \caption{Graph operations supported in TorchDrug.}
    \begin{adjustbox}{max width=0.9\textwidth}
    \begin{tabular}{lll}
        \toprule
        \bf{Class} & \bf{API} & \bf{Graph Operation} \\
        \midrule
        \multirow{7}{*}{PyTorch-like}
        & \code{data.Graph.clone} & Clone this graph \\
        & \code{data.Graph.detach} & Detach this graph \\
        & \code{data.Graph.cpu} & Move this graph to CPU \\
        & \code{data.Graph.cuda} & Move this graph to GPU \\
        & \code{data.Graph.copy\_} & Copy data from another graph \\
        & \code{data.Graph.repeat} & Repeat this graph like \code{torch.repeat} \\
        & \code{data.PackedGraph.repeat\_interleave} & Repeat this graph like \code{torch.repeat\_interleave} \\
        \midrule
        \multirow{2}{*}{Node-level}
        & \code{data.Graph.node\_mask} & Mask out some nodes from this graph \\
        & \code{data.Graph.compact} & Remove isolated nodes \\
        \midrule
        \multirow{3}{*}{Edge-level}
        & \code{data.Graph.edge\_mask} & Mask out some edges from this graph \\
        & \code{data.Graph.directed} & Return a directed version of this graph \\
        & \code{data.Graph.undirected} & Return an undirected version of this graph \\
        \midrule
        \multirow{6}{*}{Graph-level}
        & \code{data.Graph.connected\_components} & Split a graph into connected components \\
        & \code{data.Graph.split} & Split a graph into a batch of graphs \\
        & \code{data.Graph.pack} & Pack multiple graphs into a batch \\
        & \code{data.PackedGraph.graph\_mask} & Mask out some graphs from this batch \\
        & \code{data.PackedGraph.merge} & Merge some graphs into a smaller batch \\
        & \code{data.PackedGraph.unpack} & Unpack a batch into multiple graphs \\
        \midrule
        \multirow{1}{*}{Molecule}
        & \code{data.Molecule.ion\_to\_molecule} & Convert ions to molecules \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:graph_operation}
\end{table}
